Self-supervised Spatial Reasoning on Multi-View Line Drawings

Spatial reasoning on multi-view line drawings by state-of-the-art supervised deep networks is recently shown with puzzling low performances on the SPARE3D dataset. Based on the fact that self-supervised learning is helpful when a large number of data are available, we propose two self-supervised learning approaches to improve the baseline performance for view consistency reasoning and camera pose reasoning tasks on the SPARE3D dataset. For the first task, we use a self-supervised binary classification network to contrast the line drawing differences between various views of any two similar 3D objects, enabling the trained networks to effectively learn detail-sensitive yet view-invariant line drawing representations of 3D objects. For the second type of task, we propose a self-supervised multi-class classification framework to train a model to select the correct corresponding view from which a line drawing is rendered. Our method is even helpful for the downstream tasks with unseen camera poses. Experiments show that our method could significantly increase the baseline performance in SPARE3D, while some popular self-supervised learning methods cannot.

==> parts/3-scientific_experiment.tex <==
\vspace{-3.3mm}
\section{What Affects SPARE3D Performance?}
To better understand the SPARE3D tasks and why state-of-the-art deep networks have low performances, we study three potentially relevant factors: \textit{CAD model complexity, network capacity, and network structure} respectively.
For each factor, we first give a natural hypothesis about its influence on SPARE3D baseline performance. Then, we design controlled experiments to prove or disprove the hypothesis and finally obtain heuristics about both the causes of the existing baseline's low performance and potentially more effective network designs.


\textbf{Controlled experiment settings.} 
For investigating the \textit{CAD model complexity} and the \textit{network capacity} factors, we focus on the view-consistency reasoning (\textit{T2I}) and the camera-pose reasoning (\textit{I2P}) tasks on SPARE3D-ABC dataset. 
For the \textit{network structure} factor, we use both the \textit{T2I}, the \textit{I2P}, and the \textit{P2I} tasks.
We follow the same baseline settings as in~\cite{han2020spare3d}: for \textit{T2I} and \textit{P2I} tasks, we use the \textit{binary classification} baseline networks; for \textit{I2P} task, we use the \textit{multi-class classification} baseline network. The backbone network for these baseline networks are VGG-16~\cite{simonyan2014very}. We select these baseline networks since they are the best performing ones in~\cite{han2020spare3d}.
All experiments are implemented using PyTorch~\cite{PyTorch:NIPS19} and conducted on NVIDIA GeForce GTX 1080 Ti GPU.
For each experiment, we tune the hyperparameters to seek the best performance (details in the supplementary material).

\subsection{CAD model complexity}

\textbf{Motivation}: we want to study if the level of CAD model complexity affects the baseline performance for SPARE3D tasks.
It is discussed in~\cite{murty1999evaluating} that the complexity of a CAD task is associated with its difficulty for humans. However, the relationship between the CAD model complexity and the difficulty level for deep networks to solve the spatial reasoning tasks has not been fully studied.
To study the influence of CAD model complexity for deep networks, we use the number of primitives in CAD models to represent the complexity of CAD models, as discussed in~\cite{murty1999evaluating}. In practice, we use the constructive solid geometry (CSG) modeling method to generate the dataset with different numbers of primitives yet fixed primitive types and boolean operations. With the increasing number of primitives of the CSG models, the level of CAD complexity also increases.

\textbf{Hypothesis 1}: \textit{the higher level of CAD model complexity will cause lower SPARE3D baseline network performance, as long as the corresponding line drawings are still visually legible for the reasoning tasks}.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.9\columnwidth]{figs/model_complexity_examples.JPG}
	\caption{\textbf{CSG models with different number of primitives.}}
	\label{fig_cad_complexity_examples}
	\vspace{-5mm}
\end{figure}

\textbf{Experiment details.}
We use FreeCAD~\cite{riegel2016freecad} to generate a CSG model dataset with a various number of primitives. We follow the generation settings as in~\cite{han2020spare3d}. The primitives used are sphere, cube, cone, and cylinder; the Boolean operations used are intersection, union, and difference. 
For both the task \textit{T2I} and \textit{I2P}, we generate seven groups of CSG models, with primitive number \mbox{3-5}, $8$, $12$, $16$, $20$, $24$, and $30$. The \mbox{3-5} means the number of primitives making up a CAD model is $3$, $4$, or $5$. For each group, it has $4000$ models for training and $500$ models for testing. 
Exemplar line drawings rendered with CAD models composed of a different number of primitives can be seen in Figure~\ref{fig_cad_complexity_examples}. We can see that the models become visually more complex when the number of primitives increases. 

\textbf{Experiment results.}
Figure~\ref{fig_cad_complexity_result} left shows that for the \textit{T2I} task, in general, the more primitives a CSG model has, the lower the testing accuracy is, as expected in Hypothesis 1. The results for the primitive-number $12$ and $20$ are just minor variations in the experiments, which are most likely caused by the data randomness.
We think it is because when the number of primitives increases, the lines in the line drawings become denser; therefore, it is more difficult for a network to distinguish the tiny difference between candidate line drawings (see the exemplar candidate answers in Figure~\ref{fig:compare}). Thus, we call \textit{T2I} the \textit{detail-hurt task}.

However, unexpected results are shown in Figure~\ref{fig_cad_complexity_result} right, where the accuracy increases first and then decreases after the primitive number becomes more than 20. We believe it is because, within a certain range of CAD complexity, the more primitives the CAD model contains, the more visual features a network can extract for camera-pose reasoning, thus the higher testing accuracy. However, if a CAD model is too complex, the line drawings become too crowded to provide effective feature extraction and reasoning. 

We then notice that the CAD models in the SPARE3D-ABC dataset are mostly from the real world, and their complexity level is close to the CSG models with typically less than $20$ primitives. Therefore, for the SPARE3D-ABC dataset, we think more shape details can help a network in camera-pose reasoning, which we call a \textit{detail-help task}.
% For \textit{I2P} task, the result is the right figure in Figure~\ref{fig_cad_complexity_result}, we can see the line drawings using CSG with more primitives provide more visual information, which might be helpful for the reasoning. Therefore, we call the camera pose reasoning task \textit{detail help task}.


\textbf{Heuristics 1}: the experiment results show our hypothesis is not completely correct. Indeed, more shape details help the camera-pose tasks on the SPARE3D-ABC dataset but hurt the view-consistency task. Therefore, \textit{we may need different methods for them, respectively, and an effective method for \textit{T2I} task should be detail-sensitive to capture detailed differences between candidate answers}.

\begin{figure}[t]
	\centering
	\includegraphics[width=1\columnwidth]{figs/CSG_results.JPG}
	\caption{\textbf{CAD model complexity vs. test accuracy.} }
	\label{fig_cad_complexity_result}
	\vspace{-5mm}
\end{figure}

\subsection{Network capacity}

\textbf{Motivation}: we want to study if the network's capacity will affect the baseline performance for tasks on SPARE3D-ABC.
Using a large (over-parameterized) network is widely used to achieve better performance on some deep learning tasks~\cite{huang2019gpipe, tan2019efficientnet}. To increase a network's capacity, we can make the network deeper or wider without making changes to other components in the network. 

\textbf{Hypothesis 2:} \textit{a baseline network's performance will improve if the network's capacity increases}.

\textbf{Experiment details.}
With the VGG-16 network as a backbone, we define \textit{the width of the network} as the width of the last convolutional layer (the number of output channels). 
By this definition, the width of the VGG-16 network in~\cite{han2020spare3d} is $512$. In the comparative experiments, we change the width to $384$, $448$, and $1024$. The width of other convolutional layers is proportionally adapted to the final convolutional layer's width, ensuring the network's widths are changed gradually. Detailed widths of each layer for the VGG-16 backbone network with different widths can be found in the supplementary.
\textit{The depth of the network} represents the number of layers of the VGG family backbone networks. We use VGG-13, VGG-19 based backbone as in~\cite{simonyan2014very} to represent three different depths of the network.


\begin{figure}[t]
	\centering
	\includegraphics[width=1\columnwidth]{figs/width_depth_cropped.JPG}
	\vspace{-2mm}
	\caption{\textbf{Network capacity (width and depth) vs. test accuracy}. The results show that naively increasing the network capacity cannot improve the network performance on \textit{T2I} and \textit{I2P} tasks.}
	\label{fig_network_capacity}
	\vspace{-1mm}
\end{figure}

\textbf{Experiment results.}
For task \textit{T2I}, decreasing the network's width does not hurt the network's performance, although strangely, increasing the network's width leads to a decrease in the testing accuracy (Figure~\ref{fig_network_capacity} top-left). We think it is because the network with more parameters requires more data, and using the same amount of data to train networks with different widths is insufficient. For the depth control experiments, we find almost no differences among the three selected network depth values (Figure~\ref{fig_network_capacity} top-right). 
For task \textit{I2P}, neither the width nor the depth of the network can significantly improve the network's performance(Figure~\ref{fig_network_capacity} bottom).

\textbf{Heuristics 2}: our hypothesis is incorrect. In fact, merely increasing network capacities cannot improve the baseline's performances. Therefore, \textit{to improve SPARE3D performance, we need new networks or losses than only supervised classification networks with larger capacities}.

\subsection{Network structure}

\textbf{Motivation}: we want to study if the network's structure can affect the baseline performance for tasks on SPARE3D-ABC.
Changing the structure of the network is a potential way to improve the accuracy of some deep learning tasks, e.g., one famous example is to use the residual links in deep networks~\cite{he2016deep}. To find a proper structure for the view-consistency reasoning task (\textit{T2I}) and camera-pose reasoning tasks (\textit{I2P} and \textit{P2I}), we tried a lot of variants of the backbone network (all variants and the corresponding results will be shown in supplementary). We also test whether the network's performance will change if using the pre-trained parameters on Imagenet~\cite{deng2009imagenet}, inspired by~\cite{funke2020notorious}.

\textbf{Hypothesis 3:} \textit{for each SPARE3D task, a baseline network's performance will improve if we find a more proper network structure and parameter initialization}.

\textbf{Experiment details.}
We find two changes on the network that will have a consistent impact on the network's performance for all SPARE3D tasks: one is whether the network's parameters are initialized using Imagenet pre-trained parameters; another one is whether the three-view drawings (front view, right view, and top view drawings) and isometric drawings are fed to separate and independent branches of the network. We call the second one \emph{late fusion}.

\textit{Early fusion} vs. \textit{late fusion}. In the original SPARE3D paper~\cite{han2020spare3d}, the baseline backbone network treats all the input images (front, right, top view drawings, and one isometric view drawing from the candidate answers) as a whole, and it concatenates those images before sending them to the first convolutional layer. We call this way of feeding multi-view line drawings to a network as the \textit{early fusion}. In contrast, we design a network that takes the three-view drawings and the isometric view drawing as separate inputs, which means the input drawings are sent to a convolutional network that shares the \textit{same architecture} 
yet has \textit{separate network parameters}. We name this way 
of separately handling the input as the \textit{late fusion} since the extracted image features are concatenated later. Other network structures are kept the same as the baseline method in~\cite{han2020spare3d}.
Therefore, we have four experiments, which are the combination of training the network with/without Imagenet pre-trained parameters and using \textit{early fusion} or \textit{late fusion}. 

For the \textit{P2I} task, we make an extra modification of the network in the baseline method. In the original baseline method, after extracting the input images' feature vector, the feature vector is concatenated with an 8-dimensional one-hot camera-pose code. Then the concatenated vector is sent to a fully connected layer to obtain a classification probability distribution. Differently, our method extracts the feature of the composite images (F, R, T, and a candidate isometric view image) into an 8-dimensional vector as the camera-pose probability logits of the candidate isometric view. Then we select the logit corresponding to the given pose to compute the cross-entropy loss. 
We find this minor modification can effectively improve the network's performance on the \textit{P2I} task. The modification details will be given in the supplementary.


\textbf{Experiment results.}
As shown in Table~\ref{tab_network_structure}, we find that using pre-trained parameters and the \textit{late fusion} can improve the network's performance on camera-pose reasoning tasks (\textit{I2P} and \textit{P2I}). By using these tactics, the accuracy of \textit{I2P} and \textit{P2I} achieves $85.4\%$ and $72.4\%$ respectively, which is already higher than the baseline in SPARE3D.
However, the same tactics turned out to decrease the network's performance on \textit{T2I} task significantly. We leave these puzzling results for our future investigations.


\begin{table}[t]
\begin{center}
\caption{\textbf{Network architecture vs. performance.} We test four conditions, considering 1) using Imagenet pre-trained parameters or not, 2) using \textit{late fusion method} or \textit{early fusion method}. ``y/n'' indicates using the network structure or not. \textit{P2I} task uses the slightly improved network structure as previously explained.}
\begin{tabular}{ c|c|c|c|c } 
\hline
pre-train & late fusion & \textit{T2I} & \textit{I2P} & \textit{P2I}\\
\hline
n & n & \textbf{55.0} & 78.0 & 64.0\\ 
% \hline
n & y & 22.8 & 80.0 & 66.6\\ 
% \hline
y & n & 30.6 & 80.4 & 68.6\\ 
% \hline
y & y & 25.2 & \textbf{85.4} & \textbf{72.4}\\
\hline

\end{tabular}

\label{tab_network_structure}
\end{center}
\vspace{-7mm}
\end{table}

\textbf{Heuristics 3}:
based on above results, we believe: 1) \textit{a proper parameter initialization can improve baseline performances}; 2) \textit{using \textit{late fusion} or \textit{early fusion} will affect baseline performances, yet the impact depends on the task}. 
Therefore, for task \textit{T2I}, whose baseline performance is relatively lower than \textit{I2P} and \textit{P2I} (see row 1 of Table~\ref{tab_network_structure}), we still need a better method. In the next section, we will design a specialized contrastive learning method using all the above heuristics to improve the SPARE3D T2I baseline.
\vspace{-2mm}
